SoftCell: Taking Control of Cellular Core Networks

Existing cellular networks suffer from inflexible and expensive equipment, and complex control-plane protocols. To address these challenges, we present SoftCell, a scalable architecture for supporting fine-grained policies for mobile devices in cellular core networks. The SoftCell controller realizes high-level service polices by directing traffic over paths that traverse a sequence of middleboxes, optimized to the network conditions and user locations. To ensure scalability, the core switches forward traffic on hierarchical addresses (grouped by base station) and policy tags (identifying paths through middleboxes). This minimizes data-plane state in the core switches, and pushes all fine-grained state to software switches at the base stations. These access switches apply fine-grained rules, specified by the controller, to map all traffic to the appropriate addresses and tags. SoftCell guarantees that packets in the same connection traverse the same sequence of middleboxes in both directions, even in the presence of mobility. Our characterization of real LTE workloads, micro-benchmarks on our prototype controller, and large-scale simulations demonstrate that SoftCell improves the flexibility of cellular core networks, while enabling the use of inexpensive commodity switches and middleboxes.

==> controllerDesign.tex <==
\subsection{Modular Controller Design}
 %(preamble paragraph motivates the separation of service policy from traffic
 %management and low-level data-plane state) 

Our controller is akin to an operating system. It interfaces with the data plane
hardware through a switch API. It supports applications dealing with UE
authentication, subscriber billing, and service policies.  In particular, the
service policies are the main input to our controller. 

The goal of our controller is to manage traffic efficiently given
various constraints such as service policies, resource and network dynamics. Our
controller has a decision engine that makes traffic routing or rerouting
decisions in reaction to network events or policy changes. Our controller then
need to implement the routing decision using appropriate mechanisms available at
switches and communicate the implementation to the data plane switches. A
monolithic design will have to handle complexities of maintaining network state,
running a traffic management decision engine, and ensuring consistencies in low
level switch rule updates. To make it easy to handle complexities and make the
controller extensible, we would like to decouple the traffic management decision
engine from the low level implementation of traffic management decisions. Thus,
we divide our controller into two modules (or layers): traffic management layer
and mechanisms layer as shown in Figure~\ref{fig:controller}. 

\begin{figure}
\centering
\includegraphics[width=3.4in]{figures/SoftCell-controller.png}
\caption{SoftCell Controller}
\label{fig:controller}
\end{figure}

%{\bf do we need a representative example to run through each layer?}


\subsubsection{Traffic-Management Layer}
% - taking service policy and network conditions, and generating paths and
% classifiers to satisfy policy and traffic management goals 
%  (shield from how service policies are picked, and from how paths are
%   implemented and changes.  just focus on how to allocate 
%   middleboxes and paths)
%  - network conditions are compact (no per-flow state, yet application-policy
%  aware to enable intelligent decision making) 
%  - discuss what optimization techniques can be used to solve the problem?
%  mention simple case of shortest path through sequence 
%     of middleboxes along shortest network paths, or shortest paths after
%      excluding overloaded middleboxes and links. 
%  - mappings of UE events to subscriber attributes, collecting tag-level
%  measurement data, etc. 

The traffic-management layer takes service policies and network state as input;
In response to policy changes from above or network events or dynamics
(e.g. load change) from below, the decision engine computes routing and
rerouting decisions. The traffic-management layer is shielded from how service
policies are picked, and from how paths are implemented. It just focus on how to
allocate to middleboxes and paths while optimizing network wide objectives.
In order to achieve its functions, it needs to maintain network state,
associate network events with the correct subscriber attributes.

%The traffic-management layer's key functions are: (1) manage traffic effectively
%under the constraint of service policies, resource limitation and network
%dynamics (e.g. overload conditions); (2) support higher layer functions such as
%billing. The traffic management layer needs to perform its functions in real
%time and scalably. The traffic management has to be application aware to make
%intelligent decisions.

{\bf Compact and application-aware network state:} 
One key design decision is to maintain subscriber attribute based network
state. These state include UE related state and network element state. For UE
state, we can maintain per subscriber and per application traffic volume counters. See
Table~\ref{tab:uestate} for an example. For network element state, we can
% flow counters may be a bit tricky
maintain per policy traffic volume counters or unique flow
counters. See Figure~\ref{tab:netstate} for an example. These compact 
statistics is key to application-aware traffic management and supports higher
layer applications such as billing effectively. 
\begin{table}[]
\centering
\begin{tabular}{l | l | l | l}
UE ID & Location & app\_type & traffic Counter \\
\hline
1 & BS1 & video & 100 \\
\hline
2 & BS2 & other & 200 \\
\hline
\end{tabular}
\caption{An Example of UE Monitoring State}
\label{tab:uestate}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{l | l | l | l | l }
Element ID & Element Type & Policy ID & Load & capacity \\
\hline
1 & Middlebox & 1 & 100 & 200\\
\hline
2 & Link & 2 & 200 &  300 \\
\hline
3 & Switch & 2 & 400 & 500 \\
\hline
\end{tabular}
\caption{An Example of Network Element Monitoring State}
\label{tab:netstate}
\end{table}

%The traffic management layer computes paths for subscriber policy enforcement or
%for load balancing. 
%To achieve these goals, it maintains network state on
%network topology, UE location and load. For example, the load can be maintained
%per subscriber plan type or per application type or a combination of several
%attributes. 
{\bf Associating network events with subscriber attributes:}
The new flow events from access switches have a subscriber ID. The traffic
management layer uses the subscriber ID to find the subscriber attributes from
the SIB and then update the UE monitoring state. The traffic volume and unique
flow counter updates from core and gateway switches have a policy tag. The
traffic-management layer uses the policy tag to identify the right records to
update in the network element state database. 

{\bf Decision engine}: When a flow does not match any policies at the
base station (a new subscriber with a plan type not matching existing plan type
or a new subscriber with no cached subscriber attributes), the base station
generates a event similar to the OpenFlow packet\_in event to the
controller. The difference is that the message has a subscriber ID field. The
traffic management layer will first find the entry in the Subscriber Information
Base (SIB). Based on its attributes, it will find the policies from the policy
cache (not shown in the figure). If there is no match, it will send a policy
request message to the service policy application. Once the traffic management layer
gets the policy, it will compute a path for the flow based on the current
network state. The decision engine also executes when the network condition
changes such as overload conditions, and when policies change from above. 

The traffic-management layer can run \emph{ intelligent network-wide traffic
  engineering optimization algorithms}. This is enabled by the application-aware
network state. Instead of computing a shortest policy path for a new flow, the
decision engine can compute a shortest path excluding overloaded network
elements. 

{\bf Traffic management policies:}
Our application-aware network state also enables operators to specify traffic
management policies. These policies serves as an input to the decision
engine. For example, operators can specify that web traffic can be rerouted when
overload happens and video traffic should not. In case of a link failure, video
traffic should be rerouted through a pre-established backup path.  
%For example,
%the traffic management layer can relocate certain elastic traffic from a
%overloaded middlebox, base station, switch or link without rerouting inelastic
%traffic such as video streaming. 
%These are operator dependent depending on which
%resources are scarce. The traffic management layer maintains a policy cache, and
%the policies cached at each base station. 

\iffalse % not true, maintained at mechanism layer
{\bf No per switch flow table:}
% For tags, do we use soft state or hard state?
Unlike existing SDN controllers that maintain per switch flow table, SoftCell
controller does not maintain per switch flow table. Instead it maintains
network-wide policy paths. The policy paths can be un-installed for an extended
period of inactivity. The controller identifies inactivity if the periodic
traffic volume counter updates have zero value. Since core switches perform
exact match on tags, policy path addition or deletion or modification does not
affect other policy paths' forwarding decision. Since our service policies are
compact, we assume access switches cache a copy of the service policies. The
packet classifier to tag mapping table instantiates service policies. For each
policy and each UE, there will be a packet classifier. The mapping table can be
much larger than the number of service policies. Our controller does not need to
keep a copy of the mapping table. The packet classifier takes the priority of the
underlying policy. The packet classifier must contain the UE ID. So it does not
affect any other existing packet classifiers. Because of this, there is also no
need for the controller to maintain the packet classifier to tag mapping
table. Note that the packet classifier to tag mapping table has no default
mapping for all UEs. 
\fi

%{\bf what about composition? For example, one module manages monitoring and directs
%  traffic for Logging; how does it compose with the policy module?}

%{\bf who makes fine-grained load balancing decisions? 0* to firewal 1, 1* to
%  firewall 2?}

\subsubsection{Mechanism Layer}
%   - deal with edge switch capabilities -- switch table size (microflow
%   vs. wildcard in the access switch) and address space size 
%         (cache vs. embed reverse-path tags), customize to the environment while
%         shielding traffic management from details 
%         (note: we don't expect to run out of rules in the core switches
%         because of hierarchical addressing and tagging) 
%   - ensures properties (policy symmetry, loop freedom, and policy consistency),
%   transition to next two sections

The mechanism layer generates packet classifiers for access
switches. Essentially it associates a flow ID with a tag, and pushes the 
packet classifier to the edge (access switches). When
packets of the flow arrives, the packet matching a given classifier gets pushed
the appropriate tag. Other switches just perform switching based on tags.
%\emph{Note that packet classifiers are only maintained at the
%edge; other switches just perform switching based on tags}. This is a very
%simple and scalable design.
SoftCell mechanism layer shields traffic-management layer from handling low
level details of path implementation affected by switch capabilities such as
switch table size, tag address space size and from ensuring consistent updates. 
The mechanism layer has two main functions: (1) It implements the policy path
scalably in the data plane; (2) It performs consistent updates to switches.
Mechanism layers maintain switch, base station capability and flow table
size. Mechanism layer also stores the UE ID, IP and location IP address
mapping. Mechanism layer manages switch forwarding table as well.  

{\bf Path implementation:}
The mechanism layer customizes path implementation to the underlying
network environment. For example, if an access switch has enough table space,
the controller can install microflow rules. Otherwise, it can install wildcard
rules to save space. 
%Micro flow rules allows the optimization of policy paths
%during mobility (more detail in Section~\ref{sec:tag}). 
Based on the availability of tagging mechanisms such as MPLS, VLAN, the
mechanism layer will decide how to implement tags. If no MPLS mechanisms
available, it will use source port numbers to implement tags. The mechanism
layer mimimizes the switch flow table entries by intelligently aggregating
entries.   

{\bf Consistent updates:}
%To implement the policy path, we switch on tags, similar to MPLS label
%switching. We will discuss more details in Section~\ref{sec:tag}. 
Mechanism layer needs to ensure several properties. (1) loop freedom: since the
path given by the traffic management layer may not be a simple path (may contain
loops). The mechanism layer has to detect loops and break the path into multiple
simple paths. For each simple path, use labels to implement it. (2) Path symmetry:
Access switches tag outgoing packets. Return traffic must follow the same path. 
(3) Policy consistency: when a UE moves between base stations, inprogress flows
must traverse the same middleboxes.   

\emph{Note that this division of label does not affect the optimality of the
  decision engine at the traffic management layer}. Since the core switches have
sufficient table space for exact matching of our policy tags, the low level
details of switch capability does not affect the decision engine. Whether a UE
associates with a particular base station or not is determined by the radio
access networks (the base stations). Our decision engine has to take the decision
which switches handle which UE as an input. Thus, the low level details of the
switch capability does not matter to the decision engine either. 
%We discuss details of the mechanism layer in Section~\ref{sec:tag}
%and~\ref{sec:mobility}. 

%{\bf for 1000 base stations, 10 gateways and 1000 policies, this may translate
%  into 10 million tag entries in the worst case. It seems that we need an
%  optimization algorithm here.}

%Packet classifiers must be updated at the edge according to the priorities of
%the rules. For example, one may have a high priority rule which says: all
%roaming traffic go to firewall 1. A low priority rule which says: video traffic
%go to transcoder 1 and firewall 2. If the low priority rule gets updated first,
%video traffic of roaming subscribers will be sent to transcoder 1 rather than
%firewall 1. 

%{\bf discuss path consistency}


%{\bf do we allow or need to mix tagging rules with general openflow rules in
%  switches?}

